Explain3D: Explaining Disagreements in Disjoint Datasets

Data plays an important role in applications, analytic processes, and many aspects of human activity. As data grows in size and complexity, we are met with an imperative need for tools that promote understanding and explanations over data-related operations. Data management research on explanations has focused on the assumption that data resides in a single dataset, under one common schema. But the reality of today's data is that it is frequently un-integrated, coming from different sources with different schemas. When different datasets provide different answers to semantically similar questions, understanding the reasons for the discrepancies is challenging and cannot be handled by the existing single-dataset solutions. In this paper, we propose Explain3D, a framework for explaining the disagreements across disjoint datasets (3D). Explain3D focuses on identifying the reasons for the differences in the results of two semantically similar queries operating on two datasets with potentially different schemas. Our framework leverages the queries to perform a semantic mapping across the relevant parts of their provenance; discrepancies in this mapping point to causes of the queries' differences. Exploiting the queries gives Explain3D an edge over traditional schema matching and record linkage techniques, which are query-agnostic. Our work makes the following contributions: (1) We formalize the problem of deriving optimal explanations for the differences of the results of semantically similar queries over disjoint datasets. (2) We design a 3-stage framework for solving the optimal explanation problem. (3) We develop a smart-partitioning optimizer that improves the efficiency of the framework by orders of magnitude. (4)~We experiment with real-world and synthetic data to demonstrate that Explain3D can derive precise explanations efficiently.

==> deleted-others.tex <==

Canonical tuples and the mappings between them naturally form a bipartite graph. 
Each disconnected component in this bipartite graph represents two set of
tuples (and their corresponding real-world entities) that are semantically equivalent to each other.
In addition, the total impacts of the two sets of tuples in each of the connected component 
should be equal if they represents
two equivalent queries. Based on the mappings, we define \textit{equivalent} tuples and queries
as the follows.



\subsubsection*{The Explanations}
For example, 
consider query $Q_1$ and $Q_2$ in Figure~\ref{fig:comp}, 
attribute ``degree'', there are 


The existence of these
attributes may significantly increase the complexity in identifying the
matches between tuples: First, it increases the volume of the tuples 
we need to compare; Second, it increases the overall complexity of the matching
relationship between tuples. 

\iffalse
\subfigure[{\small\textbf{Mappings between tuples}}]{
		\begin{minipage}[t]{0.49\textwidth}
		\begin{tabular}{c c} 
		\multicolumn{1}{l}{Mappings:} \\ \toprule
		\hspace{1cm}$(t_i, t_j, p)$\hspace{1cm} \\\midrule
		$(m_1, d_1, 0.80)$\\
		$(m_1, d_2, 0.10)$\\
		$(m_2, d_2, 0.70)$\\
		$(m_2, d_3, 0.99)$ \\
		$(m_3, d_2, 0.90)$\\
		$(m_3, d_3, 0.70)$\\
		$(m_4, d_2, 0.90)$\\
		$(m_4, d_3, 0.60)$\\
		$(m_5, d_1, 0.75)$\\
		$(m_5, d_2, 0.30)$\\
		$(m_6, d_3, 0.15)$\\
		\bottomrule
		\end{tabular}
		\end{minipage}
	}
\fi

their matching attributes 
may not be able to uniquely identify and represent the full semantic of themselves.

we may derive such matches according to
the tuples' values in the matching attributes, which are described in attribute matching pairs
acquired directly from existing techniques.

To determine 

To determine whether two tuples match with each other, we may 
compare the values of attributes involved in the attribute matching pairs.

 their matching attributes

Matching pairs describe the semantic correlation between
two set of relevant tuples. However, their matching attributes 
may not be able to uniquely identify and represent the full semantic of themselves.
For example, tuples in Figure~\ref{fig:schools} has one matching pair 
$P = \{(\text{\textit{Major}}, \sqsubseteq, \text{\textit{Program}})\}$. 
However, the matching attribute 
``$\textit{Major}$'' in \umasstuple cannot uniquely identify themselves. 
To precisely infer the 
relationship between the tuples, we first
covert them into \textit{canonical tuples}
such that they can be fully represented by their
matching attributes. In this paper, we use functional dependencies
to decide how to convert relevant tuples into canonical forms.



\subsection{The optimal explanations}\label{sec:prob:prob}


In this paper, we target at deriving explanations over 
two semantically similar queries on two databases. 
Furthermore, we narrow down the scope of the queries
to \textit{simple aggregate queries} that do not contain
any sub-queries.
In this section, we first formally define the basic concepts
and the explanation in Section~\ref{sec:prob:basics}, then 
and formalize the explanatory problem of deriving explanation
as an optimization problem in Section~\ref{sec:prob:prob}.

\subsection{Modeling abstractions}\label{sec:prob:basics}
As shown in Example~\ref{ex:schools}, 
the input of our problem include two databases and two
semantically similar queries that operate on these two databases.
For each database and query pair, we find that only a subset of tuples
may be involved by the query and these tuples 
contribute differently to the final aggregated values (or query results).
Understanding tuples that are actually involved by the query, and 
the relationships between such tuples for the two queries (and databases) 
is essential for deriving our explanations.
Here we first introduce our modeling abstraction for tuples and their contributions in a query,
which we call \textit{relevant tuples}.


\begin{definition}[Relevant Tuples] 
 Given a pair of data-base and query $(D, Q)$, 
we first represent the query as the follows:
\[Q = (\mathcal{R}(A_1, ..., A_m), aggr, c), \]
where $\mathcal{R}(A_1, ..., A_m) = R_1 \Bowtie ... \Bowtie R_k$
is a joined relation over relations $R_i \in D$; $aggr = (f, A_i)$ is 
an aggregation, composed by an aggregate function $f$, such as COUNT or SUM, and an 
attribute name $A_i$;
and $c$ is the selection condition over attributes in the joined relation $\mathcal{R}$.
The query result is computed as $Q(D) = \Pi_{aggr}\sigma_c(\mathcal{R})$.

\smallskip

\noindent The \textbf{relevant tuples}, $T(A_1, ..., A_m, I)$, of a database and query pair, $(D, Q)$, 
is a subset of tuples 
in $\mathcal{R}$ that are selected by the condition $c$ in query $Q$. These
tuples are defined by the attribute in $\mathcal{R}$ and a \textbf{impact} value:
\[T = _{A_1, ..., A_m}\mathcal{G}_{aggr}(\sigma_{c}(\mathcal{R}))\]

Here $\sigma$ and $\mathcal{G}$ are the Selection and Group By operators in
relational algebra. The impact of a tuple $t\in T$ is a numeric value that 
measures its contribution in the final query result.
\end{definition}

In this paper, instead of the entire database, we focus on analyzing 
the relevant tuples. Considering
relevant tuples only significantly reduce the searching space of the problem.
\begin{example}\label{ex:tupleitem}
Consider the database, \ncesdb , and its SQL query $Q_2$ in Figure~\ref{fig:schools},
we may represent the query as $Q_2 = (\mathcal{R}, aggr, c)$, where $\mathcal{R}$(ID, Name, City, WebAddress, Program, BachelorDegrees) $=R_{School} \Bowtie R_{Stats}$, $ aggr = $ (SUM, BachelorDegrees), 
and $c = $ ``Name = 'University of Massachusetts-Amherst')''. There are 6 relevant tuples for \ncesdb and $Q_2$ and
their impact is determined by their \# Bach attribute values (Figure~\ref{fig:tupleitems}).
\end{example}

In order to identify the causes of the differences, we need to compare and analyze 
the semantically similar queries. However, semantically similar queries are not 
always comparable. We can hardly compare them if their relevant tuples refer
to orthogonal entities.
For example, tuples representing the number faculties per department are
not comparable with tuples representing the number of faculties per gender,
even though both of them can be used to calculate the number of faculties in a university.
Intuitively, two queries are comparable if their relevant tuples 
refer to the same real-world entities, or the same type of entities.  


Matching pairs describe the semantic correlation between
two set of relevant tuples. However, their matching attributes 
may not be able to uniquely identify and represent the full semantic of themselves.
For example, tuples in Figure~\ref{fig:schools} has one matching pair 
$P = \{(\text{\textit{Major}}, \sqsubseteq, \text{\textit{Program}})\}$. 
However, the matching attribute 
``$\textit{Major}$'' in \umasstuple cannot uniquely identify themselves. 
To precisely infer the 
relationship between the tuples, we first
covert them into \textit{canonical tuples}
such that they can be fully represented by their
matching attributes. In this paper, we use functional dependencies
to decide how to convert relevant tuples into canonical forms.


\looseness -1
Figure~\ref{fig:ctuples} (a) and Figure~\ref{fig:ctuples} (b) demonstrate the canonical tuples derived from 
databases and queries in Figure~\ref{fig:schools}. The closure
of matching attributes in \umasstuple only include two attributes, \umasstuple\textit{.Major} and \umasstuple\textit{.School}. Thus, \umassctuple include fewer tuples than \umasstuple and their impacts are accumulated accordingly.
After canonicalization, the matching attributes are able to uniquely identify the tuples in \umassctuple and can thus fully represent their semantics.

\looseness -1
Given two sets of canonical tuples on correlated or matching attributes, 
we further determine the relationship between two sets of canonical tuples
by analyzing their matching relations in the matching pairs.

\begin{definition}[Canonical tuple relationship] \label{def:rel}
Given two set of canonical tuples, $\mathbb{T}_1$ and $\mathbb{T}_2$, and
their matching pairs $P$, we determine the relationship, 
$\mathbb{R}(\mathbb{T}_1, \mathbb{T}_2)$,
between $\mathbb{T}_1$ and $\mathbb{T}_2$ as the follows.
\vspace{2mm}
\begin{itemize}[leftmargin=5mm, topsep=0mm, itemsep=0mm]  
\item \textbf{Orthogonal} ($\perp$, no mapping), if $P = \emptyset \ or\ \exists \phi_i, \phi_j \in P_\Phi, \phi_i\cup\phi_j = \{\sqsubseteq, \sqsupseteq\}$;
\item \textbf{More general} ($\sqsupseteq$, one-to-many mappings), if $\exists \phi_i \in P_\Phi, \phi_i\ is\ \sqsupseteq$;
\item \textbf{Less general} ($\sqsubseteq$, many-to-one mappings), if $\exists \phi_i \in P_\Phi, \phi_i\ is\ \sqsubseteq$;
\item \textbf{Equivalent} ($=$, one-to-one mappings), otherwise.
\end{itemize}
\end{definition}

\looseness -1
\begin{lemma}[Comparable queries]
Two semantically \\similar queries are comparable iff their canonical tuples
are \textbf{not} orthogonal.
\end{lemma}

For tuples that are not orthogonal, their corresponding queries are comparable 
as they may either refer 
to the same real-world entities
or the same type of entities with different granularity. 
When they refer to the same entity, each tuple should have
at most one matching tuple in the other side (one-to-one mapping). 
Similarly, when they refer to entities with different granularity,
a tuple that are more general may map to many tuples that are less
general, thus leads to a one-to-many mappings.
For example, based on the matching attributes, $P = \{(\text{\umasstuple.\textit{Major}}, \sqsubseteq, \text{\ncestuple.\textit{Program}})\}$, between tuples in \umassctuple and \ncesctuple,
we find that tuples in \umassctuple are less general than those in \ncesctuple, thus multiple tuples in \umassctuple may map to one in \ncesctuple. 

To acquire the mappings between two set of canonical tuples, we may 
leverage on existing entity resolution and record linkage 
techniques~\cite{davis2005establishing, benjelloun2009swoosh, whang2010entity}. 
However, such mappings are sometimes invalid if they 
fail to match with the suggested mapping requirement (one-to-to, one-to-many, or many-to-one), 
which is derived from the relationship between the canonical tuples.



\noindent Where in each mapping $(t_i, t_j, p)$, $p \in (0, 1]$ is the probability that tuple $t_i$ and $t_j$ map to each other.

\begin{example}
Figure~\ref{fig:ctuples} (c) demonstrate the mappings we acquired for canonical tuples in
Figure~\ref{fig:ctuples} (a) and Figure~\ref{fig:ctuples}(b). 
These mappings are not valid according to
Definition~\ref{def:validmapping} since the same tuple in \ncesctuple maps to
multiple tuples in \umassctuple, e.g., $p_3$ maps to both $m_4$ and $m_5$.
\end{example}

Given a set of explanations $E = (\Delta, \delta, \mathcal{M}^*)$, we
denote the
remaining tuples and mappings after reflecting $E$ on $(\mathbb{T}_1, \mathbb{T}_2, \mathcal{M})$ as $({\mathbb{T}_1}^*, {\mathbb{T}_2}^*, \mathcal{M}^*)$.
The probability of the explanations $P(E)$ is equivalent to to probability 
of the remaining tuples and mappings $P({\mathbb{T}_1}^*, {\mathbb{T}_2}^*, \mathcal{M}^*)$.
\[P(E) = P({\mathbb{T}_1}^*, {\mathbb{T}_2}^*, \mathcal{M}^*)\]


\smallskip
\xlw{
\noindent Here we assume a priori probability $\alpha$ for each tuple $t \in \mathbb{T}_1 \cup \mathbb{T}_2$ representing
the probability that $t$ is an extra tuple $P(t \notin \mathbb{T}_1 \cup \mathbb{T}_2) = \alpha$.
\begin{eqnarray}
P(\Delta) &=& \prod_{t \in \Delta}P(t \in \Delta) \prod_{t\in \mathbb{T}_1 \cup \mathbb{T}_2 \setminus \Delta} P(t \notin \Delta) \nonumber \\
 &=& \alpha^{|\Delta|} (1-\alpha)^{|\mathbb{T}_1\cup\mathbb{T}_2| - |\Delta|}
\end{eqnarray}
Note that for cases where a tuple $t \in \mathbb{T}_1 \cup \mathbb{T}_2$ appears multiple times in the original
relevant tuple sets, we may calculate $P(\Delta)$ differently by $P(\Delta) = \alpha^{|\Delta'|}(1-\alpha)^{|T_1\cup T_2| - |\Delta'|}$ with $\Delta'=\sigma_{t \in \Delta}(T_1) \cup \sigma_{t\in \Delta}(T_2)$
being the projected tuples from tuples in $\Delta \subseteq  \mathbb{T}_1 \cup \mathbb{T}_2$ to tuples in $T_1\cup T_2$.

\iffalse
Here we assume that each tuple $t \in T_1\cup T_2$ in the set of \textbf{relevant tuples} 
has a equal a priori probability $\alpha\in [0, 1]$ being an extra tuple (or tuple that should not be included). We further project tuples in $\Delta$ to the set of relevant tuples and denote the projected tuples
as $\Delta' = \sigma_{t \in \Delta}(T_1) \cup \sigma_{t\in \Delta}(T_2)$.
\fi

\smallskip

 Similarly, we denote $\beta \in [0, 1]$ as the a priori probability that a tuple $t$ has a modified impact $t.I^*$. Thus, the a priori probability that a tuple $t$ has its original impact is $1-|t.\mathcal{I}|\cdot\beta \in [0,1]$.
\begin{eqnarray}
P(\delta) &=& \prod_{t \in \delta}P(t \in \delta)\prod_{t \in \mathbb{T}_1\cup \mathbb{T}_2\setminus \delta}P(t \notin \delta) \nonumber \\
 &=& \beta^{|\delta|} \prod_{t \in \mathbb{T}_1\cup \mathbb{T}_2\setminus \delta}(1-|t.\mathcal{I}|\cdot\beta)
\end{eqnarray}
\looseness -1
One can also acquire the a priori probability of an incorrect impact explanation in a more sophisticated way such that it is calculated based on the existences of the corresponding tuples 
and the distance between the modified impact $t.I^*$ and original impact $t.I$.

\smallskip

\looseness -1
Finally, the probability $p$ for a mapping, or the probability that tuple $t_i$ and $t_j$ can be mapped together, is part of our input.
\begin{eqnarray}
P(\mathcal{M}^*) &=& \prod_{m \in \mathcal{M}^*} P(m \in \mathcal{M}^*) \prod_{m \in \mathcal{M} \setminus \mathcal{M}^*} P(m \notin \mathcal{M}^*) \nonumber \\
&=& \prod_{(t_i, t_j, p) \in \mathcal{M}^*}p\prod_{(t_i, t_j, p) \in \mathcal{M}\setminus \mathcal{M}^*}(1-p)
\end{eqnarray}

In practice, in order to improve the computation accuracy and speed up the computation, 
we calculate and later optimize the probability of a set of explanations 
in the logarithmic space. 
\begin{eqnarray}\label{eq:expprob}
&P(\Delta)' &= |\Delta| \log(\alpha) + (|\mathbb{T}_1\cup\mathbb{T}_2|-|\Delta|)\log(1-\alpha) \nonumber\\
&P(\delta)' &= |\delta| \log(\beta) + \sum_{t \in \mathbb{T}_1\cup \mathbb{T}_2\setminus \delta}\log(1-|t.\mathcal{I}|\cdot\beta) \nonumber \\
&P(\mathcal{M}^*)' &= \sum_{(t_i, t_j, p) \in \mathcal{M}^*}log(p) + \sum_{(t_i, t_j, p) \in \mathcal{M}\setminus \mathcal{M}^*}\log(1-p) \nonumber\\
&P(E)' &= P(\Delta)' + P(\delta)' + P(\mathcal{M}^*)'
\end{eqnarray}
Equation~(\ref{eq:expprob}) prioritizes explanations with fewer
number of extra tuples, fewer number of incorrect tuples, and fewer number of extra mapping 
with lower probabilities.}

==> deleted-problem2.tex <==
Essentially, the mapping relationship between a pair of queries reveals whether 
their tuples are referring to orthogonal entities, same real-world entities, or entities
belong to the same type. Using such mapping relationship, 
we determine whether two queries are comparable.
Moreover, as we will discuss later in this paper, 
we rely on this mapping relationship to reason around the database 
contents and to derive the explanations. 
Here we formally define the mapping relationship between a pair of queries as follows.

\begin{definition}[Relationship between queries] \label{def:rel}
Given two queries $Q_1$ and $Q_2$, and a set of attribute 
matches $\mathcal{M}_{attr}$,
we denote $\Phi = \{\phi | (A_i, \phi, A_j) \in \mathcal{M}_{attr}\}$ as
the matching relations in $\mathcal{M}_{attr}$
and we say $Q_1$ and $Q_2$ are:
\vspace{2mm}
\begin{itemize}[leftmargin=3mm, topsep=0mm, itemsep=0mm]  
\item \textbf{Orthogonal} ($Q_1 \perp Q_2|\mathcal{M}_{attr}$): if $\mathcal{M}_{attr} = \emptyset \ or\ \exists \phi_i, \phi_j \in \Phi, \phi_i \cup \phi_j = \{\sqsubseteq, \sqsupseteq\}$;
\item \textbf{More general} ($Q_1 \sqsupseteq Q_2|\mathcal{M}_{attr}$), if $\exists \phi \in \Phi, \phi\ is\ \sqsupseteq$;
\item \textbf{Less general} ($Q_1 \sqsubseteq Q_2|\mathcal{M}_{attr}$), if $\exists \phi \in \Phi, \phi\ is\ \sqsubseteq$;
\item \textbf{Equivalent} ($Q_1\equiv Q_2|\mathcal{M}_{attr}$), otherwise.
\end{itemize}
\vspace{2mm}
\end{definition}

\begin{definition}[Comparable queries]
Two queries, $Q_1$ and $Q_2$, are \textbf{comparable} if they are \textbf{not orthogonal}: $Q_1 \cancel{\perp} Q_2|\mathcal{M}_{attr}$.
\end{definition}
\am{I don't understand why the provenance is needed for attribute matches.
Isn't the schema all you need? If you need the data contents, it is not clear
from here why.} \xlw{I removed the provenance definition to next subsection.}


\am{I am not sure the definitions need to be this complicated at this point.
It seems that as long as the matching attributes are not empty, the queries
are comparable, and that's all you need for this definition. Is the generality
detail really necessary?} \xlw{I add a reference to later section for the purpose of this definition.}

\am{Also, provenances sounds weird.  I wouldn't use this plural form.}

\am{As I mentioned in an earlier comment, I think the structure needs to bring intuition and examples first.  This example does not heavily rely on the definitions, so it doesn't really need to come after them.}

\subsection{Explanations over comparable queries} \label{sec:prob:exp}
Two semantically similar and comparable queries may still provide
different results, just like query $Q_1$ and $Q_3$ in Figure~\ref{fig:comp}.
To understand the root causes of such differences, we need to conduct additional
reasoning over the database contents that relate to the queries. 
In this section, we first 
describe how we compare the database contents and then present our 
formalization of the explanations.


\subsubsection*{Query Provenance and Canonical Tuples}

Consider the database contents associate with 
the given queries, we find that only 
a subset of tuples are actually involved by the queries. For example, 
in Figure~\ref{fig:comp}, query 
$Q_3$ only covers a subset of tuples, representing the major 
information for University A, in database $D_3$.
While comparing and analyzing the database contents
associate with query $Q_1$ and $Q_3$, we need to exclude extra
information in the databases in order to provide precise reasoning
over the differences. Therefore, instead of the entire database, we 
focus on comparing and analyzing tuples in the provenance of the queries.
Here we model query provenance as follows.

\begin{definition}[Query Provenance]\label{def:provenance}
Given a query $Q$ over relation $R$, we present 
the \textbf{provenance} $P(A_1, ..., I)$ as a relation that
involves all tuples $\sigma_c(R)$ that satisfy the selection condition $c$ in 
relation $R$. In the provenance relation $P$, we also include the impact of a tuple
in an additional attribute $I$, which we calculate as below:
\[
t.I = \Pi_{o'}(t)
\]
Where $o'$ is \texttt{COUNT(*)} when $Q$ is a non-aggregate query, and $o'$ is
the aggregate function $o$ in query $Q$ otherwise.
\end{definition}

\am{Is there a clean way to write the provenance as a single query?}

Oftentimes, the provenance of the queries also contain attributes that
are absent from the attribute matches. In such cases, we may find some 
``duplicate'' tuples in the query provenance.
For example, in Figure~\ref{fig:comp}, we find that 
attribute ``degree'' in $D_1$ does not have a matching attribute in $D_3$.
While comparing tuples in the two databases, we may have to repeatedly 
compare and analyze tuples, representing the ``CS'' program, for multiple times.
As shown in this example, 
keeping such ``duplicate'' tuples may significantly increases the volume of tuples 
we need to compare. Therefore, to simplify the comparing process and to reduce
the size of the problem, we convert tuples in the provenance of a query into
canonical forms such that each tuple is uniquely identified by their matching
attribute values.
In particular, we use functional dependencies
to decide how we convert the tuples into canonical forms.


\begin{figure}[t]
\small
\centering     
\begin{subfigure}[b]{0.49\textwidth}
		\begin{minipage}[t]{0.49\textwidth}
		\centering
		\begin{tabular}{cl|c}
		\multicolumn{2}{l}{$T_1$:}\\ \toprule
		\textbf{rowID} & \textbf{Program}  & \textbf{\textbf{$I$}}\\ \midrule
		$m_1$ & Accounting &  1\\
		$m_2$ & CS  & 2\\	
		$m_3$ & ECE & 1\\	
		$m_4$ & EE & 1 \\
		$m_5$ & Management & 1\\
		$m_6$ & Design	& 1\\
		\bottomrule
		\end{tabular}
		\end{minipage}
\caption{Canonical tuples for $Q_1$:}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
		\begin{minipage}[t]{0.49\textwidth}
		\centering		
		\begin{tabular}{cl|c}
            \multicolumn{2}{l}{$T_2$:}\\ \toprule
            \textbf{rowID} & \textbf{Department}  & \textbf{$I$} \\
            \midrule
			$d_1$ & Business   & 2 \\ 
			$d_2$ & Engineering  & 2\\
			$d_3$ & CS & 1\\
            \bottomrule
            \multicolumn{2}{c}{} \\
            \multicolumn{2}{c}{} \\
            \multicolumn{2}{c}{} \\
        \end{tabular}
        \end{minipage}
\caption{Canonical tuples for $Q_2$:}
\end{subfigure}
\caption{Canonical tuples for query $Q_1$ and $Q_2$ in Figure~\ref{fig:comp}. $I$ denotes
the impact of the tuples.}
\label{fig:ctuples}
\end{figure}

\begin{definition}[Canonical tuples] 
Given the provenance $P$ of a query $Q$, a set of of functional dependencies $F$
over the provenance $P$, and a set of a attribute matches $\mathcal{M}_{attr}$,
we define the canonical tuples $T$ as the follows.
\[
T =
\begin{cases}
\Pi_{\mathcal{A}, I}(T),\quad &if\ T \setminus (\mathcal{A})_{F}^+ = \emptyset\\
_{\mathcal{A}}\ \mathcal{G}_{\text{\textit{SUM}}(I)}(T), &otherwise
\end{cases}
\]
\looseness -1
Where $\mathcal{A}$ is a set of matching attributes that appear in $\mathcal{M}_{attr}$; 
$_{\mathcal{A}}\mathcal{G}_{\text{SUM}(I)}$ is the Group By operation over attributes $\mathcal{A}$ with aggregate function \textit{SUM} on the impact attribute $I$; 
and $(\mathcal{A})_{F}^+$ is closure of attributes in $\mathcal{A}$ over
the set of functional dependencies $F$. 
\end{definition}

\begin{example}
Figure~\ref{fig:ctuples} demonstrates the canonical tuples for query $Q_1$ and $Q_2$ 
in Figure~\ref{fig:comp}. The closure of matching attribute in $Q_1$ does not 
include all attributes in its provenance. Thus, after canonicalization tuple with ``Program=CS''
only appears once and its impact is accumulated accordingly.
\end{example}



\subsubsection*{Equivalent Tuples}
Canonical tuples in a query may map to tuples
in another semantically similar and comparable query.
Let us take the canonical tuples for $Q_1$ and $Q_2$ in Figure~\ref{fig:ctuples},
it is highly likely that the ``CS'' program belongs to 
the ``CS'' department in University A. 
Reasoning the mappings among tuples is essential in understanding the causes
of the differences. Identifying tuples that refer to the same or correlated real-world entities
has been extensively studied as the entity resolution or record linkage
problem~\cite{davis2005establishing, 
benjelloun2009swoosh, whang2010entity, bhattacharya2006latent,domingos2004multi}. 
In this paper, we leverage these existing techniques to
acquire the initial mappings between tuples and further reason the
cause of the differences based on these acquired mappings. Without losing 
generality, we form the acquired mappings as \textit{tuple matches} as follows.

\begin{definition}[Tuple matches]\label{def:tuplematch}
Given two queries $Q_1$ and $Q_2$ and two sets of canonical tuples $T_1$
and $T_2$, we present the mappings between tuples in $T_1$ and $T_2$
as a set of \textbf{tuple matches}:
\[
\mathcal{M}_{tuple} = \{(t_i, t_j, p), ...\}
\]
Where $t_i\in T_1, t_j \in T_2$ are two tuples and $p\in(0, 1]$ is the probability
that tuple $t_i$ and tuple $t_j$ match to each other.
\end{definition}


The tuple matches we acquired are not always perfect, instead, they sometimes may 
conflict with each other. For example, in Figure~\ref{fig:comp}, existing entity resolution
techniques may decide that the ``CSE'' program in $D_2$ should be mapped to 
both the ``CS'' department and the ``Engineering'' department. 
However, it is unlikely that the same program is provided by two different departments.
In fact, the mapping relationship between queries (Definition~\ref{def:rel}) alludes
the mapping relationship between the tuples: 
For two equivalent queries, $Q_1 \equiv Q_2$, it is highly likely that
their tuples are referring to the same logical entity, thus their canonical tuples
should follow a one-to-one mapping relationship; Similarly, if one query is more
general than the other, say $Q_1 \sqsupseteq Q_2$, tuples in $Q_1$ and $Q_2$ are
likely to obey a one-to-many mapping relationship. Given a set of tuple matches,
we say that it is \textit{valid} if the matches follow the 
mapping relationship imposed by the the queries.

\begin{definition}[Valid Tuple Matches] \label{def:validtuplematch}
Given two queries, $Q_1$ and $Q_2$, their canonical tuples, $T_1$ and $T_2$, 
and a set of attribute matches $\mathcal{M}_{attr}$, 
we determine the \textbf{matching relationship} between $T_1$ and $T_2$ and the \textbf{conditions} associate
with the relationship as follows:
\vspace{2mm}
\begin{itemize}[leftmargin=3mm, topsep=0mm, itemsep=0mm]  
\item \textbf{One-to-Many} ($T_1 \leftarrow T_2$), \textbf{if} $Q_1\sqsupseteq Q_2|\mathcal{M}_{attr}$;\\
\quad Condition: $c_{\leftarrow}= \forall t_j \in T_2, |\{t_j|(t_i, t_j, p) \in \mathcal{M}_{tuple}\}| \leq 1 $
\item \textbf{Many-to-One} ($T_1 \rightarrow T_2$), \textbf{if} $Q_1\sqsubseteq Q_2|\mathcal{M}_{attr}$; \\
\quad Condition: $c_{\rightarrow}= \forall t_i \in T_1, |\{t_i|(t_i, t_j, p) \in \mathcal{M}_{tuple}\}| \leq 1 $
\item \textbf{One-to-One} ($T_1 \leftrightarrow T_2$), \textbf{if} $Q_1\equiv Q_2|\mathcal{M}_{attr}$ \\
\quad Condition: $c_{\leftarrow} \wedge c_{\rightarrow}$.
\end{itemize}

\smallskip

\noindent A set of tuple matches $\mathcal{M}_{tuple}$ is \textbf{valid} if the conditions are satisfied.
\end{definition}



\begin{figure}
\centering
\begin{subfigure}[b]{.49\linewidth}
\centering
\includegraphics[width=0.8\textwidth]{figs/tuplematches}
\caption{Acquired tuple matches}
\label{fig:tuplematches1}
\end{subfigure}
\begin{subfigure}[b]{.49\linewidth}
\centering
\includegraphics[width=0.8\textwidth]{figs/refinedmatches}
\caption{Valid tuple matches}
\label{fig:tuplematches2}
\end{subfigure}
\caption{Acquired tuple matches and valid tuple matches for tuples in Figure~\ref{fig:ctuples}. 
The acquired tuple matches are not valid as they violate the matching conditions.
The thick line, thin line, and dash line represent
tuple matches with probability in the range of $[0.75, 1], [0.25, 0.75), (0, 0.25)$ respectively.}
\label{fig:tuplematches}
\end{figure}


\begin{example}
Figure~\ref{fig:tuplematches1} shows the tuple matches we acquired for tuples $T_1$ and $T_2$ in 
Figure~\ref{fig:ctuples}. The acquired tuple matches are invalid since they are in $T_1 \rightarrow T_2$ (Many-to-One) relationship and the corresponding condition $c_{\rightarrow}$ is not satisfied. Figure~\ref{fig:tuplematches2}
shows a set of valid tuple matches where the condition is satisfied. 
\end{example}


Canonical tuples and a set of valid tuple matches naturally form a bipartite graph. 
Each disconnected component in this bipartite graph further represents two set of
tuples that are semantically equivalent to each other. For instance, $(\{m_3, m_4\}, \{d_2\}, M)$
forms a disconnected component in Figure~\ref{fig:tuplematches2}, with both sets of tuples
representing the number of programs provided by the ``Engineering'' department.
To further evaluate whether they are indeed equivalent, we also need to compare the impacts
between tuples in each of the disconnected component.
 
\begin{definition}[Equivalent tuples] \label{def:eqquery}
Given two sets of canonical tuples $T_1$ and $T_2$
and a valid set of tuple matches $\mathcal{M}_{tuple} = \{(t_i, t_j, p)\}$,
we say the canonical tuples are equivalent ($T_1\equiv T_2|\mathcal{M}_{tuple}$) iff:
\[\forall (T_1', T_2') \in \mathcal{C}, \sum_{t\in T_1'}(t.I) = \sum_{t\in T_2'}(t.I),\]
Where $\mathcal{C}$ is the collection of all connected components in the bipartite graph $G = (T_1, T_2, \mathcal{M}_{tuple})$; in each connected component, $(T_1', T_2')$, $T_1' \subseteq T_1, T_2' \subseteq T_2$.
\end{definition}

\begin{example}
Consider a valid set of tuple matches in Figure~\ref{fig:tuplematches2},
there 4 disconnected components: $(\{m_1, m_4\}, \{d_1\})$,  $(\{m_2\}, \{d_3\})$, $(\{m_3,m_4\}, \{d_2\})$,
and $(\{m_6\}, \{\})$. Among these disconnected components, the total impacts of two sets of tuples in 
$(\{m_2\}, \{d_3\})$ and $(\{m_6\}, \{\})$ are not equal, thus $T_1\cancel{\equiv} T_2|\mathcal{M}_{tuple}$.
\end{example}

\subsubsection*{The Explanations}

Intuitively, there
are two generic types of causes that may lead two similar queries providing
different results: 1). the two queries have different entity coverage, e.g., 
an entity is only covered by one of the queries; 2). the database provide
different statistics over the same entities.
\begin{example}
Let us reason around tuples in query $Q_1$ and $Q_2$ (Figure~\ref{fig:comp})
based on a set of valid tuple matches (Figure~\ref{fig:tuplematches2}).
By comparing the tuples and their impacts, we observe that there are two possible
causes that may lead to the differences: 1). The ``Design'' program
in $Q_1$ is not covered by $Q_2$; 2). The ``CS'' program is considered as
two different programs in $Q_1$ but only one in $Q_2$. The first cause indicates
that $Q_1$ and $Q_2$ have different coverage according, thus we call it
a \textbf{provenance-based explanation}; The second cause poses
that the statistics around the same entity is different, thus
we call it a \textbf{value-based explanation}. Moreover, 
the tuple matches in Figure~\ref{fig:tuplematches2} support the above
explanations and therefore serve as the \textbf{evidence}.
\end{example}

Here we formally define the two types of \textit{explanations} and 
the \textit{evidence} of the
explanations as below.

\begin{definition}[Explanations]\label{def:exp}
Given two queries $Q_1$ and $Q_2$, their canonical tuples $T_1$
and $T_2$, and a set of acquired tuple matches $\mathcal{M}_{tuple}$,
the explanations over the differences between $Q_1$ and $Q_2$ include:
\begin{itemize}[leftmargin=3mm, topsep=2mm, itemsep=0mm] 
\item \textbf{Provenance-based Explanations} ($\Delta = \{t, ...\}$):
include tuples, $t\in T_1\cup T_2$, that only are only covered by one of the queries.
\item \textbf{Value-based Explanations} ($\delta = \{t.I\mapsto t.I^*, ...\}$): 
include tuples, $t\in T_1\cup T_2$, that should have impact $t.I^*$ rather than $t.I$.
\end{itemize}
The \textbf{Evidence} for the explanations is a valid set of tuple matches:
\[\mathcal{M}_{tuple}^* \subseteq \mathcal{M}_{tuple}\]
In summary, we write a set of explanations and their evidence as:
\[E = (\Delta, \delta |\mathcal{M}_{tuple}^*).\]
Note that in our value-based explanations, we assume that all possible impacts
for each tuple is provided in advance as $t.\mathcal{I}$.
\end{definition}

\subsection{The optimal explanations}\label{sec:prob:prob}

\begin{problem}[The \probname problem]\label{def:prob}
Given two queries $Q_1$ and $Q_2$, their canonical tuples $T_1$
and $T_2$, and a set of acquired tuple matches $\mathcal{M}_{tuple}$,
our goal is to explain the differences over $Q_1$ and $Q_2$ through
a set of explanations and a corresponding evidence, 
$E = (\Delta, \delta |\mathcal{M}_{tuple}^*)$, such that:

\begin{itemize}[leftmargin=5mm, topsep=0mm, itemsep=0mm] 
\item $\mathcal{M}_{tuple}^*$ is valid;
\item $T_1^* \equiv T_2^*|\mathcal{M}_{tuple}^*$;
\item The probability of $P(E|T_1, T_2, \mathcal{M}_{tuple})$ is maximized.
\end{itemize} 
Here $T_1^* = \delta(T_1\setminus \Delta)$ and $T_2^*=\delta(T_2\setminus \Delta)$ are derived by removing tuples in the Provenance-based explanations 
and by adjusting the impacts according to the Value-based explanations.
\end{problem}

Given an instance of the \probname problem, our basic inputs include two queries ($Q_1, Q_2$) and their databases ($D_1, D_2$), and our advanced inputs include a set of attribute matches ($\mathcal{M}_{attr}$) and a set of tuple matches ($\mathcal{M}_{tuple}$), acquired from two blackboxes based on existing schema matching and entity resolution techniques. The acquired attribute matches help us derive the 
mapping relationship between the queries, and the acquired tuples
matches support our further reasoning in explaining the differences.
Based on these provided inputs, our goal is to derive a set of explanations 
over an evidence, $E = (\Delta, \delta |\mathcal{M}_{tuple}^*)$, that fully
explain the differences and obtain the maximum posteriori probability.

From Bayesian inference, the posteriori probability of the explanations, $P(E|T_1, T_2, \mathcal{M}_{tuple})$,
is proportional to the likelihood $P(T_1, T_2, \mathcal{M}_{tuple}|E)$ and the probability $P(E)$.
\begin{eqnarray} \label{eq:prob}
P(E|T_1, T_2, \mathcal{M}_{tuple})  \propto P(T_1, T_2, \mathcal{M}_{tuple} | E) P(E)
\end{eqnarray}

In this paper, we assume explanations are independent to each other and all have 
a uniform probability: $\forall e \in E, P(e) = \gamma$. Based on our assumption, we write $P(E)$ as:
\begin{eqnarray} \label{eq:prob:e}
P(E) = \prod_{e\in E} \gamma = \gamma ^{|\Delta + \delta|}
\end{eqnarray}

Next, we consider $P(T_1, T_2, \mathcal{M}_{tuple} | E)$. For simplicity, 
we assume that tuples and tuple matches are independent to each other,
thus, $P(T_1, T_2, \mathcal{M}_{tuple} | E) = P(T_1, T_2|E)P(\mathcal{M}_{tuple}|E)$.
Let us denote $\mathcal{T} = T_1 \cup T_2$, for each tuple $t \in \mathcal{T}$,
we assume a priori probability $\alpha \in (0, 1]$ representing
the probability that $t$ is included by both queries:
\[ P(t|t \notin \Delta) = \alpha, P(t|t\in \Delta) = 1- \alpha.\] 
Similarly, we assume another a priori probability $\beta \in (0, 1]$ representing 
a tuple $t$ has correct impact $t.I$:
\[P(t.I|t\notin \delta, t \notin \Delta) = \beta, \\ 
P(t.I|t\in \delta, t \notin \Delta) = 1-\beta \\
P(t.I|t \notin \Delta) = 0\]
Based on the a priori probabilities, we calculate $P(T_1, T_2|E)$ as the follows.
\begin{eqnarray}\label{eq:tprob}
P(T_1, T_2|E) &=& \prod_{t\in \mathcal{T}}P(t) P(t.I) \nonumber \\
				&=& \alpha^{|\mathcal{T}| - |\Delta|}(1-\alpha)^{|\Delta|}\beta^{|\mathcal{T}| - |\delta|}(1-\beta)^{|\delta|} 
\end{eqnarray}
\looseness -1
For simplicity,
we represent $\alpha$, $\beta$ as fixed values for all tuples, however, one can always set different probabilities for distinct tuples and impacts.

\smallskip

We next calculate the probability of the evidence $P(\mathcal{M}_{tuple}|E)$.
For a tuple match $m = (t_i, t_j, p)$, the probability that tuple $t_1$ and $t_j$ is a match is provided
as part of the input, thus:
\[P(m|m\in \mathcal{M}_{tuple}) = p, P(m|m\notin \mathcal{M}_{tuple}^*) = 1-p \]
Based on the given probabilities, we calculate $P(\mathcal{M}_{tuple}|E)$ as:

\begin{eqnarray}\label{eq:mprob}
P(\mathcal{M}_{tuple}|E) &=& \prod_{m \in \mathcal{M}_{tuple}} P(m) \nonumber \\
 						  &=& \prod_{m \in \mathcal{M}_{tuple}^*} p \prod_{\substack{m \in \mathcal{M}_{tuple} \\ m \notin \mathcal{M}_{tuple}^*}} (1-p)
\end{eqnarray}

In practice, in order to improve the computation accuracy and efficiency, 
we calculate and later optimize the probability of a set of explanations 
in the logarithmic space. 
\begin{align}
P(E)' =& (|\Delta| + |\delta|)\log(\gamma)\nonumber \\
P(T_1, T_2|E)' =& (|\mathcal{T}| - |\Delta|)\log(\alpha) + |\Delta|\log(1-\alpha) + \nonumber \\ 
&(|\mathcal{T}| - |\delta|)\log(\beta) + |\delta|\log(1-\beta) \label{eq:tupleprob}\\
P(\mathcal{M}_{tuple}|E)' =& \sum_{m \in \mathcal{M}_{tuple}^*}\log(p) + \sum_{\substack{m \in \mathcal{M}_{tuple} \\ m \notin \mathcal{M}_{tuple}^*}} \log(1-p)  \label{eq:matchprob} \\
P(E|T_1, T_2, \mathcal{M}_{tuple})' = & P(E)' + P(T_1, T_2|E)' + P(\mathcal{M}_{tuple}|E)' \label{eq:eprob}
\end{align}

According to Equation~(\ref{eq:tupleprob})$\sim$(\ref{eq:eprob}), 
we find that our objective function $P(E)$ prioritizes explanations with fewer tuples in both
of the provenance-based and value-based explanation, and prefers keeping tuple matches with 
higher probabilities in the evidence.

\begin{theorem}
The \probname problem (Problem~\ref{def:prob}) is NP-complete.
\end{theorem}

\input{content/npproof}



==> summarize.tex <==
\noindent \textbf{Summarized Explanations.~}
We further summarize the derived explanations by Data X-Ray~\cite{wang2015data},
which significantly reduces the number of explanations and makes
the explanations easier to understand. We demonstrate the size of original
explanations and the size of summarized explanations is shown in Figure~\ref{fig:summarize}.

\begin{figure}
\centering
{\small \it
\begin{tabular}{c|c|c|c}
\toprule
\multicolumn{2}{c|}{\textbf{Academic datasets}}  & \multicolumn{2}{c}{\textbf{IMDB datasets}} \\\midrule
\textit{UMass vs. NCES} & \textit{OSU vs. NCES} & \textit{Template Q1} & \textit{Template Q2}\\\hline
$ 59 \rightarrow 10$ & $106 \rightarrow 13$ & $1608 \rightarrow 28$ & $3561 \rightarrow 38$\\\bottomrule
\end{tabular} 
}
\caption{Number of explanations after the summarization stage.}
\label{fig:summarize}
\end{figure}

